OpenDraco: A Platform for Engineering and Experimenting with Configurable Multi-Agent Architectures for Software Engineering

Experimenting with LLM-based multi-agent systems (MAS) involves an iterative cycle of modeling configurations, executing and evaluating them, comparing results, and refining system designs. Existing approaches provide limited end-to-end support for this experimentation lifecycle. We present OpenDraco, an open-source platform that integrates these activities into a single workflow. OpenDraco represents agents, prompts, tools, models, parameters, and communication topology in exportable, versioned JSON specifications, translated into executable LangGraph workflows supporting different interaction structures. Users can modify and re-evaluate configurations using local or cloud-based LLMs. We instantiate OpenDraco for automated program repair (APR) and evaluate a sequential baseline and seven reconstructed configurations on synthetic and real-world SWE-bench Lite issues. The results reveal substantial cost differences among configurations with similar repair outcomes, while the baseline resolves 12 of 77 SWE-bench issues using open-source LLMs. Additional proof-of-concept tasks illustrate applicability beyond APR. OpenDraco supports iterative experimentation with heterogeneous MAS configurations, enabling researchers to examine their outcomes and costs within a common environment. Demonstration video: https://youtu.be/278sOR4lBEk.

==> macros.tex <==
% ============================================================
%  macros.tex -- project-wide LaTeX macros for the OpenDraco
%  ICSE tool-demonstration paper.
% ============================================================

% ---- TODO marker -------------------------------------------
\newif\ifshowtodo
\showtodotrue % set to \showtodotrue to show all TODO markers
% \showtodofalse % set to \showtodofalse to hide all TODO markers


\newcommand{\TODO}[1]{%
  \ifshowtodo
    {\color{red}\textbf{[TODO: #1]}}%
  \fi
}

% ---- Product / concept shorthands --------------------------
\usepackage{comment}
\newcommand{\toolname}{\textit{OpenDraco}\xspace}
% Unitalicized variant for section headings: IEEEtran sets titles in small
% caps, and small-caps+italic (T1/ptm/m/scit) does not exist in Times.
\newcommand{\toolnameplain}{OpenDraco\xspace}
\newcommand{\swebench}{\textit{SWE-bench}\xspace}
\newif\iffirstLLM \firstLLMtrue
\newif\iffirstMAS \firstMAStrue
\newif\iffirstAPR \firstAPRtrue
\newcommand{\resetacronyms}{\firstLLMtrue\firstMAStrue\firstAPRtrue}

% First-use acronyms: expand to ``Full Name (ABBR)'' on first use, then ``ABBR'' after.
\newcommand{\LLM}{\iffirstLLM Large Language Model (LLM)\global\firstLLMfalse\else LLM\fi\xspace}
\newcommand{\LLMs}{\iffirstLLM Large Language Models (LLMs)\global\firstLLMfalse\else LLMs\fi\xspace}
\newcommand{\MAS}{\iffirstMAS Multi-Agent System (MAS)\global\firstMASfalse\else MAS\fi\xspace}
\newcommand{\MASs}{\iffirstMAS Multi-Agent Systems (MAS)\global\firstMASfalse\else MAS\fi\xspace}
\newcommand{\APR}{\iffirstAPR Automated Program Repair (APR)\global\firstAPRfalse\else APR\fi\xspace}

% ---- Cross-reference shorthands ----------------------------
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}

% ---- Code / identifier formatting --------------------------
% \code sets identifiers/paths in typewriter. \texttt{} is never hyphenated,
% so a long path or identifier is a rigid box that forces under/overfull lines
% in the narrow IEEE column. We locally redefine \_ so every underscore offers
% a zero-width break point (no hyphen is inserted, per URL/path convention).
\let\codeus\_
\makeatletter
% Walk the argument, splitting on "/" and inserting a break after each one.
% A sentinel "/" is appended so the delimited pattern always matches; the
% recursion stops when the remainder is empty.
\def\code@slash#1/#2\@nil{%
  #1%
  \def\code@rest{#2}%
  \ifx\code@rest\@empty\else/\allowbreak\code@slash#2\@nil\fi}
\DeclareRobustCommand{\code}[1]{%
  \texttt{\def\_{\codeus\allowbreak}\code@slash#1/\@nil}}
\makeatother

% ---- Author review comments -------------------------------
% All annotation macros honor \ifshowtodo: with \showtodofalse the
% comments/done-notes vanish (clean PDF), and \xxrewrites keep their
% text but drop the color. Toggle everything with \showtodotrue/false.
\newcommand{\mmcomment}[1]{\ifshowtodo{\color{teal}\texttt{MM: #1}}\fi}
\newcommand{\xfcomment}[1]{\ifshowtodo{\color{blue}\texttt{XF: #1}}\fi}
\newcommand{\vmcomment}[1]{\ifshowtodo{\color{violet}\texttt{VM: #1}}\fi}

\newcommand{\mm}[1]{{\color{teal}\itshape #1}}
\newcommand{\mmrewrites}[1]{\ifshowtodo{\color{teal}\itshape #1}\else #1\fi}
\newcommand{\xfrewrites}[1]{\ifshowtodo{\color{blue}\itshape #1}\else #1\fi}
\newcommand{\vmrewrites}[1]{\ifshowtodo{\color{violet}\itshape #1}\else #1\fi}

% ---- Resolved (done) comments ------------------------------
\newcommand{\mmdone}[1]{\ifshowtodo{\color{teal}\texttt{\sout{MM: #1}}}\fi}
\newcommand{\xfdone}[1]{\ifshowtodo{\color{blue}\texttt{\sout{XF: #1}}}\fi}
\newcommand{\vmdone}[1]{\ifshowtodo{\color{violet}\texttt{\sout{VM: #1}}}\fi}

% ---- Results-table helpers ---------------------------------
\newcommand{\inline}[1]{\code{#1}}
\newcommand{\SWEBench}{\swebench}

% \resolvedboxes{11011} -> five small squares, one per synthetic
\newcommand{\resolvedboxfilled}{\textcolor{green!55!black}{\rule[-0.1ex]{1.3ex}{1.3ex}}}
\newcommand{\resolvedboxempty}{\textcolor{black!18}{\rule[-0.1ex]{1.3ex}{1.3ex}}}
\makeatletter
\def\resboxloop#1{%
  \ifx\relax#1%
  \else
    \ifnum#1=1 \resolvedboxfilled\else\resolvedboxempty\fi\kern1pt
    \expandafter\resboxloop
  \fi}
\makeatother
\newcommand{\resolvedboxes}[1]{\resboxloop#1\relax}
